TALC: Time-Aligned Captions for Multi-Scene Text-to-Video Generation

Most of these text-to-video (T2V) generative models often produce single-scene video clips that depict an entity performing a particular action (e.g., 'a red panda climbing a tree'). However, it is pertinent to generate multi-scene videos since they are ubiquitous in the real-world (e.g., 'a red panda climbing a tree' followed by 'the red panda sleeps on the top of the tree'). To generate multi-scene videos from the pretrained T2V model, we introduce a simple and effective Time-Aligned Captions (TALC) framework. Specifically, we enhance the text-conditioning mechanism in the T2V architecture to recognize the temporal alignment between the video scenes and scene descriptions. For instance, we condition the visual features of the earlier and later scenes of the generated video with the representations of the first scene description (e.g., 'a red panda climbing a tree') and second scene description (e.g., 'the red panda sleeps on the top of the tree'), respectively. As a result, we show that the T2V model can generate multi-scene videos that adhere to the multi-scene text descriptions and be visually consistent (e.g., entity and background). Further, we finetune the pretrained T2V model with multi-scene video-text data using the TALC framework. We show that the TALC-finetuned model outperforms the baseline by achieving a relative gain of 29% in the overall score, which averages visual consistency and text adherence using human evaluation.

==> files/qualtative_examples.tex <==
% \begin{figure*}[h]
% \centering
% {\includegraphics[width=0.9\textwidth]{images/talc_examples_v2.pdf}}
% \caption{{\bf Examples of multi-scene video generation using the \name framework.} \my{ Our proposed method, \name, enhances scene-level alignment between text and video, facilitating the generation of videos with seamless transitions between textual descriptions while preserving visual consistency. The first two rows are generated using Lumiere \cite{bar2024lumiere} and the last two rows use ModelScope \cite{wang2023modelscope}.}}
% \label{fig:talc_examples}
% \end{figure*}



==> files/related_work_backup_august11.tex <==
\section{Related Work}
\label{sec
}

\paragraph{Text-to-Video Generative Modeling.}
The field of text-to-video (T2V) synthesis has significantly evolved from its inception with models like VGAN~\cite{vondrick2016generating} and MoCoGAN~\cite{tulyakov2018mocogan}, leveraging the foundational technologies of GANs~\cite{creswell2018generative} and VAEs~\cite{doersch2016tutorial} to produce concise, single-scene videos. The narrative depth was further expanded through transformer-based architectures such as CogVideo~\cite{hong2022cogvideo} and VideoGPT~\cite{yan2021videogpt}, enhancing the complexity of video content yet remaining within the confines of single scenes. The advent of diffusion models, exemplified by Imagen Video~\cite{ho2022imagenvideo}, marked a notable advancement in T2V synthesis. Despite these strides, the challenge of creating multi-scene videos that reflect the complexity of the physical world~\cite{acharya2018towards,vondrick2016generating,bruce2024genie} remains. \blue{While some recent works like Phenaki~\cite{villegas2022phenaki} have explored generating videos of arbitrary length with a focus on temporal coherence, direct comparisons are challenging as the code is not publicly available. Additionally, works like VideoDirectorGPT~\cite{lin2023videodirectorgpt} and DirecT2V \cite{hong2023direct2v} have introducted a zero-shot approach to multi-scene video generation, which differs from our approach as we incorporate fine-tuning for enhanced performance. Other methods, such as Gen-l-Video~\cite{wang2023gen}, use a denoising process to iteratively refine video content in order to generate consistent videos by aggregating overlapping short video clips. StreamingT2V~\cite{henschel2024streamingt2v} employs a streaming-based approach, utilizing an auto-regressive process, where video content is generated continuously and sequentially. However, our work, \name, extends the capabilities of T2V models to multi-scene storytelling, filling a crucial gap in the synthesis landscape.}

\paragraph{Image-to-Video Animation.}
The exploration of multi-scene video generation, innovative methods such as Lumiere~\cite{bar2024lumiere} and Make-a-Video~\cite{singer2022make} have employed a two-step process, transforming text to images and then animating these images into videos. While these approaches have advanced visual quality, they often fall short in weaving seamless multi-scene narratives. This limitation is echoed in the work of Emu Video~\cite{girdhar2023emu} \blue{and Dynamicrafter~\cite{xing2023dynamicrafter}}, which underscores the difficulty of achieving narrative coherence across multiple scenes. \name focuses on direct generation of multi-scene narratives from textual prompts aiming for a narrative flow and visual consistency across scenes.

\paragraph{Multi-Scene Video Generation.}
The pursuit of multi-scene T2V synthesis has been furthered by recent innovations like Phenaki~\cite{villegas2022phenaki} and Stable Video Diffusion~\cite{blattmann2023stable}, which have explored new frontiers in video generation from textual prompts and the scaling of latent diffusion models, respectively. Additionally, Dreamix~\cite{molad2023dreamix} and Pix2Video~\cite{ceylan2023pix2video} have broadened the scope of diffusion models, applying them to video editing and animation. \blue{There are also works that provide better methods for frames concatenations~\cite{lu2023vdt,voleti2022mcvd}}. Despite these advancements, the task of generating videos that convey coherent narratives across multiple scenes remains formidable, highlighted by recent works such as VideoPoet~\cite{kondratyuk2023videopoet}, ModelScope~\cite{wang2023modelscope} and Make-A-Scene~\cite{gafni2022make}. \name tackles this task and offers a framework produces videos spanning multiple scenes. We also introduce nuanced evaluation approach. This approach integrates both automated assessments and human evaluations to rigorously gauge the quality and narrative coherence of the generated content, evaluating text adherence, object consistency and background consistency, contributing to the ongoing refinement of T2V synthesis.

==> files/related_work_backup_sept_1.tex <==
\section{Related Work}
\label{sec
}

Generating videos from textual descriptions, particularly those spanning multiple scenes with coherent narratives, is a challenging task in computer vision. This section explores related work in text-to-video generation, highlighting the limitations addressed by our approach, \name. 

\paragraph{Text-to-Video Generative Modeling:} 
The field of text-to-video (T2V) synthesis has witnessed significant progress, transitioning from early models like VGAN~\cite{vondrick2016generating} and MoCoGAN~\cite{tulyakov2018mocogan} based on GANs~\cite{creswell2018generative} and VAEs~\cite{doersch2016tutorial} for generating short, single-scene videos to more advanced transformer-based architectures such as CogVideo~\cite{hong2022cogvideo} and VideoGPT~\cite{yan2021videogpt} that enhance video content complexity, yet still remain confined to single-scene generation. Diffusion models like Imagen Video~\cite{ho2022imagenvideo} signify a notable advancement, but the creation of multi-scene videos that realistically capture the nuances of the physical world~\cite{acharya2018towards,vondrick2016generating,bruce2024genie} remains a significant challenge.

Recent research has explored generating longer videos, but these approaches come with limitations. Phenaki~\cite{villegas2022phenaki} aims for arbitrary length videos and focuses on temporal coherence, but its evaluation is hindered by the lack of publicly available code.  \blue{VideoDirectorGPT~\cite{lin2023videodirectorgpt}, DirecT2V~\cite{hong2023direct2v} and Free-bloom~\cite{huang2024free}, while tackling multi-scene generation, employ a zero-shot approach, contrasting with our method that incorporates fine-tuning for enhanced performance. Other approaches, such as Gen-l-Video~\cite{wang2023gen}, utilize iterative denoising to aggregate overlapping short video clips and create longer, consistent videos. However, we observed that Gen-l-Video mainly generates videos with a maximum of two scenes, while our method produces videos with up to four distinct scenes. StreamingT2V~\cite{henschel2024streamingt2v} adopts a streaming auto-regressive process for continuous video generation. While these methods showcase progress in long video generation, they often struggle to maintain visual consistency and strict adherence to multi-scene textual descriptions, crucial for compelling narrative storytelling.}

\paragraph{Image-to-Video Animation:} 
Several innovative methods, including Lumiere~\cite{bar2024lumiere} and Make-a-Video~\cite{singer2022make}, generate multi-scene videos through a two-step process: first generating images from text and then animating these images to create video sequences.  However, these approaches often fall short in maintaining narrative consistency across different scenes, leading to disjointed storylines.  Works like Emu Video~\cite{girdhar2023emu} \blue{and Dynamicrafter~\cite{xing2023dynamicrafter}} further exemplify the inherent difficulty of achieving smooth transitions and coherent storytelling across multiple scenes using image-to-video animation techniques.

\paragraph{Multi-Scene Video Generation:} 
Directly tackling multi-scene T2V synthesis, recent work such as Phenaki~\cite{villegas2022phenaki} and Stable Video Diffusion~\cite{blattmann2023stable} push the boundaries of text-driven generation by exploring novel approaches and scaling latent diffusion models.  Dreamix~\cite{molad2023dreamix} and Pix2Video~\cite{ceylan2023pix2video} leverage diffusion models for video editing and animation, \blue{while research on frame concatenation techniques, such as MCVD~\cite{voleti2022mcvd} and VDT~\cite{lu2023vdt}, focuses on improving temporal consistency in longer videos. Despite these advancements, creating multi-scene videos that accurately reflect complex narratives with high visual fidelity remains a difficult task, as evidenced by the ongoing research efforts in projects like VideoPoet~\cite{kondratyuk2023videopoet}, ModelScope~\cite{wang2023modelscope}, and Make-A-Scene~\cite{gafni2022make}.}

\blue{\name directly addresses the challenge of multi-scene video generation, aiming to enhance both visual consistency and text adherence across scenes. Unlike existing zero-shot methods, \name leverages fine-tuning on a curated multi-scene video dataset rather than zero-shot approaches. To rigorously evaluate \name's effectiveness, we propose a comprehensive evaluation protocol that includes both human evaluation and automated assessments using GPT-4V. This approach ensures a robust and reliable measure of narrative coherence in generated multi-scene videos.} 



% \paragraph{Text-to-Video Generative Modeling.}
% The field of text-to-video (T2V) synthesis has significantly evolved from its inception with models like VGAN~\cite{vondrick2016generating} and MoCoGAN~\cite{tulyakov2018mocogan}, leveraging the foundational technologies of GANs~\cite{creswell2018generative} and VAEs~\cite{doersch2016tutorial} to produce concise, single-scene videos. The narrative depth was further expanded through transformer-based architectures such as CogVideo~\cite{hong2022cogvideo} and VideoGPT~\cite{yan2021videogpt}, enhancing the complexity of video content yet remaining within the confines of single scenes. The advent of diffusion models, exemplified by Imagen Video~\cite{ho2022imagenvideo}, marked a notable advancement in T2V synthesis. Despite these strides, the challenge of creating multi-scene videos that reflect the complexity of the physical world~\cite{acharya2018towards,vondrick2016generating,bruce2024genie} remains. \blue{While some recent works like Phenaki~\cite{villegas2022phenaki} have explored generating videos of arbitrary length with a focus on temporal coherence, direct comparisons are challenging as the code is not publicly available. Additionally, works like VideoDirectorGPT~\cite{lin2023videodirectorgpt} and DirecT2V \cite{hong2023direct2v} have introducted a zero-shot approach to multi-scene video generation, which differs from our approach as we incorporate fine-tuning for enhanced performance. Other methods, such as Gen-l-Video~\cite{wang2023gen}, use a denoising process to iteratively refine video content in order to generate consistent videos by aggregating overlapping short video clips. StreamingT2V~\cite{henschel2024streamingt2v} employs a streaming-based approach, utilizing an auto-regressive process, where video content is generated continuously and sequentially. However, our work, \name, extends the capabilities of T2V models to multi-scene storytelling, filling a crucial gap in the synthesis landscape.}

% \paragraph{Image-to-Video Animation.}
% The exploration of multi-scene video generation, innovative methods such as Lumiere~\cite{bar2024lumiere} and Make-a-Video~\cite{singer2022make} have employed a two-step process, transforming text to images and then animating these images into videos. While these approaches have advanced visual quality, they often fall short in weaving seamless multi-scene narratives. This limitation is echoed in the work of Emu Video~\cite{girdhar2023emu} \blue{and Dynamicrafter~\cite{xing2023dynamicrafter}}, which underscores the difficulty of achieving narrative coherence across multiple scenes. \name focuses on direct generation of multi-scene narratives from textual prompts aiming for a narrative flow and visual consistency across scenes.

% \paragraph{Multi-Scene Video Generation.}
% The pursuit of multi-scene T2V synthesis has been furthered by recent innovations like Phenaki~\cite{villegas2022phenaki} and Stable Video Diffusion~\cite{blattmann2023stable}, which have explored new frontiers in video generation from textual prompts and the scaling of latent diffusion models, respectively. Additionally, Dreamix~\cite{molad2023dreamix} and Pix2Video~\cite{ceylan2023pix2video} have broadened the scope of diffusion models, applying them to video editing and animation. \blue{There are also works that provide better methods for frames concatenations~\cite{lu2023vdt,voleti2022mcvd}}. Despite these advancements, the task of generating videos that convey coherent narratives across multiple scenes remains formidable, highlighted by recent works such as VideoPoet~\cite{kondratyuk2023videopoet}, ModelScope~\cite{wang2023modelscope} and Make-A-Scene~\cite{gafni2022make}. \name tackles this task and offers a framework produces videos spanning multiple scenes. We also introduce nuanced evaluation approach. This approach integrates both automated assessments and human evaluations to rigorously gauge the quality and narrative coherence of the generated content, evaluating text adherence, object consistency and background consistency, contributing to the ongoing refinement of T2V synthesis.

==> files/video_generation_methods.tex <==
\begin{figure*}[t]
\centering
{\includegraphics[width=\textwidth]{images/video_generation_methods.pdf}}
\caption{{{\bf Examples of multi-scene video generation baselines.} (a) Generating video on the merged descriptions, leads to a poor text-video alignment. (b) Generating videos for the individual text descriptions and concatenate them temporally, leads to a lack of background consistency. (c) Our approach (TALC) enhances the scene-level text-video alignment and maintains background consistency. \hb{lets remove this (keep this in appendix instead) and add better qualitative examples here. we don't need to show merge captions/videos in the main text. just focus on the quality of TALC.}}}
\label{fig:video_generation_methods}
\end{figure*}
